Beyond Additive Composition: Interventional Modeling of State-Dependent Cross-Degradation Responses for Composite Image Restoration

Composite image restoration aims to recover images corrupted by multiple coexisting degradations. Existing methods predominantly decompose composite corruptions into individual factors, relying on these isolated priors to guide restoration. However, coexisting degradations are inherently interdependent: the manifestation of one degradation dynamically shifts with the states of others, inducing non-additive interactions that factor-wise paradigms fail to capture. To bridge this gap, we formulate state-dependent cross-degradation responses and propose PROBE, an interventional framework that explicitly models how coexisting degradations influence one another. Specifically, we first construct unified degradation axes by aligning visual and textual degraded-clean offsets. Along these axes, a calibrated coordinate head estimates current degradation states, while bidirectional feature perturbations are injected to probe cross-coordinate responses under the current states. Contrasting these responses with corresponding intensity-matched single-degradation references quantifies intrinsic non-additive deviations, allowing the resulting response descriptors and state coordinates to jointly guide restoration. For comprehensive evaluation, we introduce SCD-15, a new benchmark covering all 15 nonempty combinations of four degradation factors at three severity levels. Experiments demonstrate that PROBE achieves state-of-the-art performance on the CDD-11, AWMM-100K, and SCD-15 composite restoration datasets using a compact model with modest GPU memory requirements.

==> sec/front_performance.tex <==
\begin{figure}[!t]
  \captionsetup{margin=0pt}
  \centering
   \includegraphics[width=1\linewidth]{sec/figures/params_vs_psnr.png}

   \caption{Restoration quality and resource costs on CDD-11. PSNR is plotted against parameter count (left axis) and memory usage (right axis). Positions closer to the upper right indicate higher restoration quality and lower resource costs. PROBE improves PSNR over the baseline by 1.59\,dB, with only 0.62\,M additional parameters (3.6\%) and 9\,MiB additional memory (7.6\%).}
   \label{fig:onecol}
\end{figure}

